Understanding Incentivized Mobile App Installs on Google Play Store

"Incentivized" advertising platforms allow mobile app developers to acquire new users by directly paying users to install and engage with mobile apps (e.g., create an account, make in-app purchases). Incentivized installs are banned by the Apple App Store and discouraged by the Google Play Store because they can manipulate app store metrics (e.g., install counts, appearance in top charts). Yet, many organizations still offer incentivized install services for Android apps. In this paper, we present the first study to understand the ecosystem of incentivized mobile app install campaigns in Android and its broader ramifications through a series of measurements. We identify incentivized install campaigns that require users to install an app and perform in-app tasks targeting manipulation of a wide variety of user engagement metrics (e.g., daily active users, user session lengths) and revenue. Our results suggest that these artificially inflated metrics can be effective in improving app store metrics as well as helping mobile app developers to attract funding from venture capitalists. Our study also indicates lax enforcement of the Google Play Store's existing policies to prevent these behaviors. It further motivates the need for stricter policing of incentivized install campaigns. Our proposed measurements can also be leveraged by the Google Play Store to identify potential policy violations.

==> Makefile <==
.PHONY: quick paper.pdf all clean

TEX = main
FIGS =
PSFIGS = $(FIGS:.pdf=.ps)

all: quick
ps:  $(TEX).ps
pdf: $(TEX).pdf
dvi: $(TEX).dvi

clean:
	$(RM) *.out *.aux *.log *.bbl *.blg *~ \#*\# *.toc *.idx *.eps dummy
	$(RM) $(patsubst %.tex, %.ps, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.dvi, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.pdf, $(wildcard *.tex))

quick: *.tex
	# python2.7 latex_export_example.py
	pdflatex main.tex

paper.pdf: *.tex shehroze.bib Makefile
	# python2.7 latex_export_example.py
	pdflatex main.tex
	bibtex main.aux
	pdflatex main.tex
	pdflatex main.tex


==> old-commands.tex <==
\mathchardef\Gamma="0100 \mathchardef\Delta="0101
\mathchardef\Theta="0102 \mathchardef\Lambda="0103
\mathchardef\Xi="0104 \mathchardef\Pi="0105
\mathchardef\Sigma="0106 \mathchardef\Upsilon="0107
\mathchardef\Phi="0108 \mathchardef\Psi="0109
\mathchardef\Omega="010A

\newcommand{\ovspace}[1]{\vspace{#1}}

\newcommand{\outline}[1]{}%{\textbf{#1}}

\newcommand{\dl}{\mbox{$\, [ \hspace*{-1.5pt} [\,$}}
\newcommand{\dr}{\mbox{$\, ] \hspace*{-1.5pt} ]\:$}}
\newcommand{\da}{\mbox{$\, A \hspace*{-6.75pt} A \,$}}
%\newcommand{\drightarrow}{\mbox{$\rightarrow \hspace*{-8pt} \rightarrow$}}

\newcommand{\BA}{\mbox{${\bm{a}}$}}
%\newcommand{\BB}{\mbox{${\bm{c}}$}}
\newcommand{\BC}{\mbox{${\bm{c}}$}}
\newcommand{\BD}{\mbox{${\bm{d}}$}}
\newcommand{\BE}{\mbox{${\bm{e}}$}}
\newcommand{\BO}{\mbox{${\bm{o}}$}}
\newcommand{\BP}{\mbox{${\bm{p}}$}}
\newcommand{\BQ}{\mbox{${\bm{q}}$}}
\newcommand{\BR}{\mbox{${\bm{r}}$}}
\newcommand{\BV}{\mbox{${\bm{v}}$}}
\newcommand{\BL}{\mbox{${\bm{l}}$}}
\newcommand{\BI}{\mbox{${\bm{i}}$}}
\newcommand{\BH}{\mbox{${\bm{h}}$}}
\newcommand{\BS}{\mbox{${\bm{s}}$}}
\newcommand{\BB}{\mbox{${\bm{k}}$}}

\newcommand{\wrapbox}[1]{\framebox{\begin{tabular}{c}#1\end{tabular}}}
\newcommand{\CodeIn}[1]{{\small\texttt{#1}}}
\newcommand{\Section}[1]{Section~\ref{sec:#1}}
\newcommand{\SFigure}[2]{Figure~\ref{fig:#1}(#2)}

\usepackage{rotating}
\usepackage{cite}
\usepackage{xspace}
\usepackage{url}
\usepackage{graphicx}
\usepackage{latexsym}
\usepackage{amssymb}
\usepackage{amsfonts}
%\usepackage{times}
\usepackage{psfrag}
%\usepackage{algorithm2e}
\usepackage{wrapfig}
\usepackage{comment}
%packages for algorithms
%\usepackage{algorithm}
%\usepackage{algorithmic}
\usepackage{alltt}
\usepackage{color}

\newtheorem{defn}{Definition}[section]
\newtheorem{exmp}{Example}[section]
\newtheorem{thrm}{Theorem}[section]
\newtheorem{prop}{Proposition}[section]
\newtheorem{lemm}{Lemma}[section]
\newtheorem{obsv}{Observation}[section]
\newtheorem{corr}{Corollary}[section]

%\addtolength{\textheight}{.23in} \addtolength{\textwidth}{.15in}
%\addtolength{\topmargin}{-.23in}
%\addtolength{\oddsidemargin}{.1in}
%\addtolength{\evensidemargin}{.1in}

\newtheorem{thm}{Theorem}
\newtheorem{dfn}{Definition}
\newtheorem{lem}{Lemma}
\newtheorem{cor}{Corollary}
\newcommand{\ie}{\emph{i.e.}\xspace}
\newcommand{\eg}{\emph{e.g.}\xspace}
\newcommand{\etc}{\emph{etc.}\xspace}
\newcommand{\etal}{\frenchspacing{}\emph{et al{.}}\xspace}
%\newcommand{\etal}[1]{{\sl et al.{#1}}}

%\newcommand{\thm}[1]{Theorem~\ref{thm:#1}}
%\newcommand{\lem}[1]{Lemma~\ref{lemma:#1}}
%\newcommand{cor}[1]{Corollary~\ref{cor:#1}}
\newcommand{\fac}[1]{Fact~\ref{fact:#1}}
\newcommand{\Table}[1]{Table~\ref{tab:#1}}
\newcommand{\Figure}[1]{Figure~\ref{fig:#1}}

%\theoremstyle{plain}
\newtheorem{property}{Property}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{theorem}{Theorem}[section]

%\theoremstyle{definition}
\newtheorem{notation}{Notation}
\newtheorem{Definition}{Definition}[section]

%\theoremstyle{remark}
\newtheorem{fact}{Fact}[section]
\newtheorem{observation}{Observation}[section]
\newtheorem{insight}{Insight}[section]

\newcommand{\Comment}[1]{}

\renewcommand\floatpagefraction{0.999}
\renewcommand\topfraction{0.999}
\renewcommand\bottomfraction{0.999}
\renewcommand\textfraction{0.001}
\setcounter{totalnumber}{5}

